Timed Automata for Modelling Caches and Pipelines

In this paper, we focus on modelling the timing aspects of binary programs running on architectures featuring caches and pipelines. The objective is to obtain a timed automaton model to compute tight bounds for the worst-case execution time (WCET) of the programs using model-checking techniques.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{R.J. van Glabbeek, J.F. Groote \& P. H\"ofner (Eds.):
Workshop on\\
Models for Formal Analysis of Real Systems (MARS 2015)\\
EPTCS 196, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.196.4}{10.4204/EPTCS.196.4}}
\pdfoutput=1

